On the Robustness of Bayesian Neural Networks to Adversarial Attacks

Vulnerability to adversarial attacks is one of the principal hurdles to the adoption of deep learning in safety-critical applications. Despite significant efforts, both practical and theoretical, training deep learning models robust to adversarial attacks is still an open problem. In this paper, we analyse the geometry of adversarial attacks in the large-data, overparameterized limit for Bayesian Neural Networks (BNNs). We show that, in the limit, vulnerability to gradient-based attacks arises as a result of degeneracy in the data distribution, i.e., when the data lies on a lower-dimensional submanifold of the ambient space. As a direct consequence, we demonstrate that in this limit BNN posteriors are robust to gradient-based adversarial attacks. Crucially, we prove that the expected gradient of the loss with respect to the BNN posterior distribution is vanishing, even when each neural network sampled from the posterior is vulnerable to gradient-based attacks. Experimental results on the MNIST, Fashion MNIST, and half moons datasets, representing the finite data regime, with BNNs trained with Hamiltonian Monte Carlo and Variational Inference, support this line of arguments, showing that BNNs can display both high accuracy on clean data and robustness to both gradient-based and gradient-free based adversarial attacks.

==> Sections/AdvRobBNNs.tex <==
\subsection{A Symmetry Property of Neural Networks}
\label{sec:AdvRobBNNs}

%\LL{Improve and increase the discussion}

\noindent
Before considering the BNN case, in Proposition \ref{Proposition:ExtensionLemmaForNNs} below we show a symmetry property of neural networks: given a  neural network, we can always find an infinitely-wide NN that has the same loss but opposite orthogonal gradient. %proving that for any $\x\in $ the orthogonal component of the expected loss gradient vanishes for an infinitely-wide BNN, i.e. under some assumptions $ \langle\nabla^\perp_\x L(\x,\w)\rangle_{p\left(\w\vert D\right)}$ converges to zero. 
In order to prove this result, we first introduce Lemma \ref{extension_lemma}, which is a generalization of the submanifold extension lemma  %(Lemma 5.34 in \cite{leeintroduction})
and a key result we leverage. It proves that any smooth function defined on a submanifold $\mathcal{M}$ can be extended to the ambient space, in such a way that the choice of the derivatives orthogonal to the submanifold is arbitrary. 

%\ap{I don't understand, first it is reported as a result we extend from Lee et al., then it's reported as a result from Anders et al?}
\begin{lemma}[\cite{anders2020fairwashing}]\label{extension_lemma}
Let $T_\x\mathcal{M}$ be the tangent space of $\mathcal{M}$ at a point $\x\in\mathcal{M}$. Let $V=\sum_{i=\mathrm{dim}\left(\mathcal{M}\right)+1}^d v^i \partial_i$ be a conservative vector field along $\mathcal{M}$ which assigns a vector in $T_\x\mathcal{M}^\perp$
for each $\x\in\mathcal{M}$. For any smooth function $f^{true}:\mathcal{M}\to\mathbb{R}$ there exists a smooth extension $F:X\to\mathbb{R}$ such that 
$$ F|_\mathcal{M} = f^{true},
$$
where $F|_\mathcal{M}$ denotes the restriction of $F$ to the submanifold $\mathcal{M}$, and such that the derivative of the extension $F$ is 
\begin{align*}
    \nabla_\x F(\x)=(\nabla_1 f^{true}(\x), \ldots, &\nabla_{\mathrm{dim}\left(\mathcal{M}\right)} f^{true}(\x),\\ &v^{\mathrm{dim}\left(\mathcal{M}\right)+1}(\x), \ldots, v^{d}(\x))
\end{align*}
for all $\x\in\mathcal{M}$.
\end{lemma}
\noindent
Notice that in Lemma \ref{extension_lemma}, in $\nabla_\x F(\x)$, we pick the local coordinates at $\x\in \mathcal{M}$, such that the first set of components parametrises the data manifold. We stress that, as $\mathcal{M}$ is smooth, this is without any loss of generality \citep{leeintroduction}. 
Lemma \ref{extension_lemma}, together with the universal approximation capabilities of NNs \citep{hornik1991approximation}, is employed in Proposition \ref{Proposition:ExtensionLemmaForNNs} to show that for any possible value $\mathbf{v}$ of the orthogonal gradient to the data manifold in a point,  there exists at least two (possibly not unique) different weight vectors that achieve zero loss and have orthogonal gradients respectively equal to $\mathbf{v}$ and $-\mathbf{v}$.

%an infinitely-wide NN $f$ converges uniformly to a function achieving zero loss and having that orthogonal gradient.
%it is always possible to select two sets of weights, $\w_1$ and $\w_2$, such that $f(\cdot,\w_1)$ and $f(\cdot,\w_2)$ have same loss and orthogonal gradients of the loss at a point $\x$ on the data manifold. Specifically, we build an extension of the loss function outside of the data manifold, with suitable derivatives in the orthogonal components, and we leverage results on the global convergence of overparameterized neural networks to approximate the extension of the prediction function with an overparametrised neural network.

\iffalse

\begin{proposition}
\label{Proposition:ExtensionLemmaForNNs}
Let $f^{true}: \mathcal{M} \to \mathbb{R}^k$ be a smooth function  and $f$ be a neural network with smooth activation functions and last layer of size $L$.
Then, for any $\mathbf{v}\in \mathbb{R}^{\mathrm{dim}\left(X \right)-\mathrm{dim}\left(\mathcal{M}\right)}$, $\x\in \mathcal{M}$ and $\epsilon>0$ there exist $\bar{L}$ such that if $L>\bar{L}$, then there exists set of weights $\w_L$ such that  
$$  \sup_{\mathbf{x}' \in \mathcal{M}}|| f(\mathbf{x}',\w_1)|_{}-f^{true}(\mathbf{x}')||_{\infty}\leq \epsilon$$ $$||\nabla_\x^\perp f(\x,\w_L)-\mathbf{v}||_{\infty}\leq \epsilon.$$
%That is, $f(\cdot,\w_1)$ and $f(\cdot,\w_2)$ coincide on $$, but have opposite orthogonal loss gradients in $\x$. 
\end{proposition}

\begin{proof}
Let's consider a neural network $f(\cdot,\w_L)$, where $L$ is the size of the last layer. Since $\nabla_\x^\perp f$ is continuous in any compact set $\mathcal{C}\subset X$ around $\x$, %in a compact set $\mathcal{C}\subset X$, i.e. an $\tilde{f}:X\to\mathbb{R}^k$ such that $\tilde{f}|_\mathcal{C}\approx\nabla_\x^\perp f(\cdot,\w_L)|_\mathcal{C}$. Then $\tilde{f}$ is continuous on a compact set, thus 
it is limited in $\mathcal{C}$. Therefore, for any  $\mathbf{v}\in \mathbb{R}^{\mathrm{dim}\left(X \right)-\mathrm{dim}\left(\mathcal{M}\right)}$ % the norm $||\tilde{f}(\x)-\mathbf{v}||_{\infty}$ is bounded and we obtain $$||\nabla_\x^\perp f(\x,\w_L)-\mathbf{v}||_{\infty} \leq ||\nabla_\x^\perp f(\x,\w_L)-\tilde{f}(\x)||_{\infty}+||\tilde{f}(\x)-\mathbf{v}||_{\infty} \leq \epsilon.$$
$$||\nabla_\x^\perp f(\x,\w_L)-\mathbf{v}||_{\infty} \leq \epsilon.$$
\LL{I do not see why the above holds. In particular, what makes the gradient of the neural network to converge to $\mathbf{v}$ for any $\epsilon>0$? %Also, why you need a continuous approximation of the gradient, if this is already continuous (assuming smooth activation functions)?\gc{we don't need it, maybe it's better to say it explicitly in the assumptions}
}

From Lemma \ref{extension_lemma} we know that there exists a smooth extension $F$ of $f^{true}$ 
to the embedding space such that 
$\nabla_\x^\perp F(\x) =\mathbf{v}$
for any $\x\in \mathcal{M}$.  
%\gc{If the orthogonal gradients of $f$ are limited in a closed convex set around $\x$, then there exists $\v$ such that $$||\nabla_x^\perp f(\x,\w_L)-\mathbf{v}||_{\infty}\leq \epsilon $$.} 
We can then rely on the universal approximation capabilities of NNs \citep{hornik1991approximation} to show  for any $\epsilon>0$ there exists a finite size  $\bar{L}\in\mathbb{N}$ of the last layer of $f$ such that for any $L\geq\bar{L}$ there exists a set of weights $\w_L$ for which
$$
\sup_{\x\in \mathcal{M}}||f(\x,\w_L)-F(\x)||_{\infty} \leq \epsilon$$
for any $\x\in\mathcal{M}$. This proves the theorem, because $F\big|_\mathcal{M}\equiv f^{true}$.

%%%%%%%%%% PREVIOUS VERSION %%%%%%%%%% 

% From Lemma \ref{extension_lemma} we know that there exists a smooth extension $F$ of $f^{true}$ 
% to the embedding space  such that 
% $\nabla_\x^\perp F(\x) =\mathbf{v}$
% for any $\x\in \mathcal{M}$. We can then rely on the Universal Approximation Theorem \citep{cybenko1989approximation} to show  for any $\epsilon>0$ there exists a finite size  $L\in\mathbb{N}$ of the last layer of $f$ such that  there exists a set of weights $\w_1$ for which
% $$
% \sup_{\x\in \mathcal{M}}| F(\x)-f(\x,\w_1) |_{\infty} < \epsilon$$
% for any $\x\in\mathcal{M}$.
% Finally, to conclude, we can employ Theorem 7.17 in \cite{rudin1964principles}
% that guarantees that if $f(\x,\w_1)$ converges to $F(\x)$ uniformly on any closed convex set $\mathcal{C}\subseteq X$ then for any $\x \in \mathcal{C}$ also the partial derivatives wrt $\x$ converge. \LL{That theorem also requires that the derivates of the NN converges uniformly on $\mathcal{C}$. How do you show that or are you using another version of the Theorem?}

\end{proof}
A straightforward consequence of  Proposition \ref{Proposition:ExtensionLemmaForNNs} is the following corollary.

\fi

\begin{proposition}\label{Proposition:ExtensionLemmaForNNs}
 Consider a NN $f$ with $M+1$ layers, last hidden layer of size $n_M$ and an input $\x\in \mathcal{M}$. Then, in the limit of $n_M\to \infty$ (size of last hidden layer going to infinity), for any smooth function ${f}^{true}:\mathcal{M} \to \mathbb{R}$ and vector $\mathbf{v}\in \mathbb{R}^{\mathrm{dim}\left(X \right)-\mathrm{dim}\left(\mathcal{M}\right)}$, there exist  $\w_1, \w_2$
 such that
 \begin{align}
 f(\cdot,\w_1) |_{\mathcal{M}} = {f}^{true}  =f(\cdot,\w_2) |_{\mathcal{M}} \label{eq:restriction}\\
\nabla_\x^\perp f(\x,\w_1)=\mathbf{v}=-\nabla_\x^\perp f(\x,\w_2).\label{eq:opposite_grads}
\end{align}
%[scrivilo for any smooth functions]
%For a given measure $\mu,$ e.g. Lebesque measure, let $L(\w)=\int_{} L(\x,\w) d\mu(\x), $ be the integral of the loss over  $$. Assume that for any $\w, $ the supremum of $L(\w)$ is $M\leq \infty$ is equal to some constant $M<\infty$, i.e., $\sup_{\w}L(\w)= M$. Consider a NN $f$ of size $N$ and an input $\x\in $. Then, in the limit of $N\to \infty,$ for any $0\leq l < M$ and $\textbf{v}\in \mathbb{R}^{d-\text{dim}(D)}$ there exist weight set $\w_1, \w_2$ achieving loss $l$ and such that
%$$\nabla_\x^\perp L(\x,\w_1)=\mathbf{v}=-\nabla_\x^\perp L(\x,\w_2),$$
%that is, both $\w_1$ and $\w_2$ have same and have opposite orthogonal gradients in $\x$.
\end{proposition}
\begin{proof}
From Lemma \ref{extension_lemma} we know that there exist smooth extensions $F^+$ and $F^-$ of $f^{true}$ 
to the embedding space such that 
$\nabla_\x^\perp F^+(\x) =\mathbf{v}=-\nabla_\x^\perp F^-(\x)$.
As a consequence, to conclude the proof it suffices to apply Theorem 3 in \citep{hornik1991approximation} that guarantees that infinitely-wide neural networks are \emph{uniformly 1-dense} on compacts in $\mathcal{C}^1(X)$, under the assumptions of smooth, bounded, and non-constant activation functions. 
Specifically, for any $F\in \mathcal{C}^1(X)$ and $\epsilon>0$, for any compact $X'\subseteq X$ there exists a set of weights $\w$ s.t.
\begin{align*}
    \max\Big\{ \sup_{\x\in X'}&|| F(\x)-f(\x,\w)||_{\infty},\\ &\sup_{\x\in X'}|| \nabla F(\x) - \nabla f(\x,\w) ||_{\infty} \Big\} \leq \epsilon.
\end{align*}
As $F^+,F^- \in \mathcal{C}^1(X)$, this concludes the proof.


%As $\bar{f}$ is smooth, Lemma \ref{extension_lemma} guarantees that it can be extended on the ambient space to smooth functions ${F^+}$ and $F^{-}$ that are equal to $\bar{f}$ on $\mathcal{M}$ and have gradients in the direction orthogonal to $\mathcal{M}$ in $\x$ equal to $\mathbf{v}$ and $-\mathbf{v}$. Finally, to conclude we employ Proposition \ref{Proposition:ExtensionLemmaForNNs} to guarantee uniform convergence of both functions and their gradients for $L\to\infty.$
\end{proof}
\noindent
Note that by the chain rule, the gradient of the loss is proportional to the gradient of the NN. As a consequence, 
Proposition \ref{Proposition:ExtensionLemmaForNNs} guarantees that,
for infinitely-wide NNs, for any set of weights achieving the minimum loss, %\ap{I think not just any loss, I think it needs to be the minimum loss.}
then there exists another set of weights with same loss and opposite orthogonal gradient of the loss w.r.t.\ the input. This suggests that by averaging over these configurations of the weights one can achieve a robust model that has vanishing expected orthogonal gradient. In the next Section, in Theorem \ref{thm:main} we show this is indeed the case. However, we should already emphasize  that such a result does not hold by simply averaging the set of weights w.r.t.\ any distribution. Intuitively, for this result to hold, it is required that each set of weights achieving a given gradient value has the same measure as the set of weights with the same loss and opposite orthogonal gradient value.




\section{Adversarial Robustness via Bayesian Averaging}
\label{sec:adv_robustness_bayesian_averaging}
%\LL{Need to assume somewhere that the true underlying function is in the RKHS of the NN. (similar than in Rotskoff)}
%\LL{Need to connect better with the story and avoid to introduce things twice. For instance, definition of BNNs and uninformative prior should be in background section}
%\LL{Need to be formal in here and in how we define everything.}
%\LL{Equations for the BNN and GP kernel are commented in here. They should be introduced in Section 2}


We are now ready to state Theorem \ref{thm:main}, where we show that under the assumption of a flat prior, the posterior of an infinitely-wide BNN achieving zero loss has vanishing orthogonal gradients. 
%\LL{We may want to assume that $f^true$ is in the RKHS of the NN.}
\begin{theorem}\label{thm:main}
    Let $f(\x,\w)$ be an infinitely-wide BNN trained on a data set $D_N$ composed by $N$ data points  with true underlying function $f^{true}:\mathcal{M} \to \mathbb{R}$.
    Assume that:
    \begin{itemize}
        \item The prior is flat.%, i.e., for any $H\subseteq \mathcal{C}^{\infty}$ with  and $g \in \mathcal{C}^{\infty}$ it holds that $\int_{H}p_f(f(\cdot,\w))df = \int_{g+ H}p_f(f(\cdot,\w))df,$  where $g+ H=\{ g + f \mid f \in H \}$ is the pointwise addition of $g$ to $H.$
        \item For $N\to\infty$ the posterior distribution of the BNN  converges weakly to a distribution that achieves zero loss with probability $1$, i.e., %\LL{Here we need to use big $P$ becasue we are talking about probability measure, small $p$ is the density function.}
        $$ P( f(\cdot,\w) | D_N )\xrightarrow{d} P( f \mid D_{\infty} ) ,$$
        where $P( f \mid D_{\infty} )$ is such that  
        \begin{equation}\label{eq:zero_loss}
            P\Big(\sup_{\x \in \mathcal{M}} |f(\x) - f^{true}(\x) |=0 \,\Big|\, D_{\infty}\Big)=1.
        \end{equation} %\LL{Need to check if this is more than what we need}
    \end{itemize}
Then, for any $\x\in \mathcal{M}$ it holds that
    \begin{equation}
       \langle\nabla_\x^\perp f(\x,\w)\rangle_{p(f(\cdot,\w)\mid{D_N)}}\to 0.
    \label{eq:expected_gradient}
    \end{equation}
\end{theorem}

\begin{proof}
Without any loss of generality assume that $\mathrm{dim}\left(X\right)-\mathrm{dim}\left(\mathcal{M}\right)=1$.\footnote{In the case that $\mathrm{dim}\left(X\right)-\mathrm{dim}\left(\mathcal{M}\right)>1$, because of the linearity of the partial derivatives, any component of $\langle\nabla_\x^\perp f(\x)\rangle_{p(f \mid {D_{\infty})}}$ can be treated analogously to the case $\mathrm{dim}\left(X\right)-\mathrm{dim}\left(\mathcal{M}\right)=1$. } 
Consider the operator $$\mathcal{G}_\x:f\mapsto\nabla_\x^\perp f(\x),$$ which is linear and bounded under the boundeness assumption on the derivatives of $f$. % and acts on functions $\mathcal{C}(X,\mathbb{R}^n)$. %almost surely on smooth functions, i.e., $f\in \mathcal{C}^{\infty}$ by the smoothness assumption of the NN activation functions.\LL{This is not generally true, becasue a limit sequence of smooth functions is not necessarily smooth (it may be even just continuous). So, need to see if continuity is enough (otherwise need to consider the limit space of neural networks)} 
%on functions belonging to the (reproducing kernel Hilbert) limit space of infinitely-wide networks \citep{}.
By the Portmanteau theorem, $\mathcal{G}_\x$ preserves weak convergence, hence
\begin{equation}
       \langle\nabla_\x^\perp f(\x,\w)\rangle_{p(f(\cdot,\w)\mid {D_N)}}\to \langle\nabla_\x^\perp f(\x)\rangle_{p(f \mid {D_{\infty})}}.
    \end{equation}
Then, to prove Equation \eqref{eq:expected_gradient} it is enough to show that
$$ \langle\nabla_\x^\perp f(\x)\rangle_{p(f \mid {D_{\infty})}} = 0.$$ 
%Given a fixed point $\x\in$ we consider the set $\mathcal{G}^{-1}(\mathbf{v})=\{f \mid \nabla_\x f(\x)=\mathbf{v}\}$ of all functions with a fixed value $\mathbf{v}\in\mathbb{R}^d$ of the gradient in $\x$. 
In order to do that, we proceed as follows. By definition of expectation we have that %it is convenient to express $ \langle\nabla_\x^\perp f(\x)\rangle_{p(f \mid {D_{\infty})}}$ in spherical coordinates as follows.%, where with an abuse $P(\mathcal{G}^{-1}(\mathbf{v})|D_\infty)$ is the density representing the probability that a function sampled from $P(f \mid {D_{\infty})}$ has gradient $\textbf{v}$:% \LL{Nota per me: questo spazio di probabilita in realta è semplicemente la distribuzione del gradiente in un punto rispetto la posterior. Quindi quello che diciamo ė che la density è constante. VOglio capire se è formale abbastanza o se dovremmo lavorare direttamente con spazi di funzione di misura non-zero}%\LL{I would add some intuition behind the various steps}
\begin{align}
\nonumber
\langle\nabla_\x^\perp f(\x)\rangle_{p(f \mid {D_{\infty})}}
    &= \int_{\mathbf{v}\in \mathbb{R}^{}}\displaylimits \mathbf{v} \, p{(\nabla_\x^\perp f(\x)=\mathbf{v}|D_\infty)}d\mathbf{v}
    \\ 
    \nonumber =\int_{\mathbf{v}\in \mathbb{R}_{> 0}}\displaylimits& \mathbf{v} \, p(\nabla_\x^\perp f(\x)=\mathbf{v}|D_\infty)d\mathbf{v} \,+
    \\ 
    &\, \int_{\mathbf{v}\in \mathbb{R}^{}_{< 0}}\displaylimits \mathbf{v} \, p{(\nabla_\x^\perp f(\x)=\mathbf{v}|D_\infty)}d\mathbf{v}  
    \label{eqn:Average}.
\end{align}
%\noindent%\\
%    &=\sum_{i=1}^{N} \int_{\mathbf{v}\in [v_{i-1},v_i]}\displaylimits \mathbf{v} \, p{(\nabla_\x^\perp f(\x)=\mathbf{v}|D_\infty)}d\mathbf{v} \,+\, \int_{\mathbf{v}\in [-v_{i},-v_{i-1}]}\displaylimits \mathbf{v} \, p{(\nabla_\x^\perp f(\x)=\mathbf{v}|D_\infty)}d\mathbf{v}. 
   % &=\int\displaylimits_{\mathbf{v}\in\mathbb{R}^d}  \mathbf{v}\, {P(\mathcal{G}^{-1}(\mathbf{v})|D_\infty)}d\mathbf{v}\\
 %   &=\int\displaylimits_{r\geq 0} r \int\displaylimits_{\mathbf{u} \in S^{d-1}} \mathbf{u}\,p{(\nabla_\x^\perp f(\x)=r\mathbf{u}\mid D_\infty)} d\mathbf{u}dr,
%    \label{eqn:IntegralDecomposition}

%\gc{why do we always have a counter image of $\mathbf{v}$ in (7) -> (8)?} \lb{BECAUSE OF THE EXTENSION THEOREM, WHICH IS TELLING YOU THAT YOU CAN EXTEND A FUNCTION ON THE MANIFOLD TO HAVE AN ARBITRARY (MAYBE CONTINUOUS, WE NEED TO SPECIFY BETTER CONDITIONS ON $\mathbf{v}(\x)$). But in a single point $\x$, you can extend to an arbitrary vector. }
%\LL{Ma non mi serve sfera, visto che è la media di una random variable con distribuzione uniforme. Quindi va a zero}
%where $\mathbf{u}$ is a vector belonging to the unitary sphere $S^{d-1}$  in $\mathbb{R}^d$. 
%where $v_0,...,v_N$ is any partition of $\mathbb{R}^{d}_{\geq 0}$\footnote{Note that as $\nabla_\x^\perp f(\x)$ is bounded with probability 1 by assumption we can consider closed intervals}.

%\gc{why do we have the decomposition only on positive or negative values for all components of $\mathbf{v}$? what about mixed sign?}\LL{THis integral is supposed to be for any component of the Jacobian. Let me specify.}
%where $\mathbb{R}^{\bar{d}}_{> 0}$ and $\mathbb{R}^{\bar{d}}_{< 0}$ denote vectors in $\mathbb{R}^{\bar{d}}$ whose components are, respectively, all positive or negative.

If we now can show that for any $\mathbf{v}\in \mathbb{R}^{}$ and $\epsilon \in \mathbb{R}^{}_{>0}$, $P(\nabla_\x^\perp f(\x)\in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon] \mid D_\infty):=\int_{[\mathbf{v}-\epsilon,\mathbf{v}+\epsilon]}{p{(\nabla_\x^\perp f(\x)=v\mid D_\infty)}}d{v}$ %\gc{why don't we take the integral between -v and v directly?}\LL{Because to conclude I need to show that the density is constant, but in order to prove it, I need to use events of non-zero measure and then rely on the general form of the theorem of calculus} 
is constant w.r.t.\ $\mathbf{v}$, then this guarantees that Eqn \eqref{eqn:Average} is zero. In fact, by application of the fundamental theorem of calculus, the above implies that for any $\mathbf{v},$ $p(\nabla_\x^\perp f(\x) =\mathbf{v}\mid D_\infty)=p(\nabla_\x^\perp f(\x)=-\mathbf{v} \mid D_\infty)$ almost surely (i.e.\ with probability $1$), hence terms in Eqn  \eqref{eqn:Average} cancel out. We prove that  $P(\nabla_\x^\perp f(\x)\in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon] \mid D_\infty)$ is constant wrt $\mathbf{v}$ in what follows. %the integral on the sphere is identically zero, hence we can conclude the proof. \LL{This should hold because gradient is bounded and continuous. Hence, function is Reimann integrable.}

By assumption it holds that any $f\sim P(\cdot|D_\infty)$ is such that $\forall\bar{\x}\in\mathcal{M}, f(\bar{\x})=f^{true}(\bar{\x})$ almost surely. Hence, to conclude, %in order to prove that $\int_{[\mathbf{v}-\epsilon,\mathbf{v}+\epsilon]}{p{(\nabla_\x^\perp f(\x)=k,\mid D_\infty)}}dk$ is constant wrt  $\mathbf{v}$, 
being our prior invariant to translations (see Definition \ref{Def:UninformativePrior}), it is enough to show that for any $\mathbf{v},\mathbf{v}'$ sets 
\begin{align*}
    F_{\mathbf{v}} = \{g \in &\mathcal{F}~:~\forall \bar{\x} \in \mathcal{M},\\ \, &g(\bar{\x})=f^{true}(\bar{\x}) \wedge \nabla_\x^\perp g(\x) \in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon]\}\\
    F_{\mathbf{v}'} = \{g \in &\mathcal{F} ~:~\forall \bar{\x} \in \mathcal{M},\\ \,  &g(\bar{\x})=f^{true}(\bar{\x}) \wedge \nabla_\x^\perp g(\x) \in [\mathbf{v}'-\epsilon,\mathbf{v}'+\epsilon] \}
\end{align*}
are equal up to a translation. %, i.e., for any set of points $\x_1,...x_{M},$ there exists a function $\bar{f}\in \mathcal{F}$ such that \begin{align*}\{\big(f(\x_1),...f(\x_M) \big)& \mid  f\in F_{\mathbf{v}}   \}=\\
%&\{\big(f(\x_1)+\bar{f}(\x_1),...f(\x_M) +\bar{f}(\x_M)\big) \mid f\in F_{\mathbf{w}}   \}.\end{align*}
This can be shown as follows.
 Using Lemma \ref{extension_lemma} we extend $f^{true}$ 
%we fix a function $f$ on $$ such that $\sup_{\bar{\x}\in  } f^{true}(\bar{\x})-f(\bar{\x})= 0$ almost surely. Lemma \ref{extension_lemma} allows us to extend $f$ 
to a smooth function $f_{\mathbf{v}}$ in $X$ %(in fact, we need to extend it only on an embedding of $\mathcal{M}$ in $\mathbb{R}^d$),
such that its orthogonal gradient in $\x \in \mathcal{M}$ equals $\mathbf{v}$, i.e.  $\nabla_\x^\perp f_{\mathbf{v}}(\x) = \mathbf{v}.$ %\gc{Here we know that the parallel components of the gradient are zero and we are only extending the orthogonal components as $\mathbf{v}(x)$, right? Just to make it clear. YES, WE ASK THE FUCNTION $f$ TO HAVE ZERO LOSS ON THE DATA MANIFOLD}
Then, because of the linearity of the gradient operator, any  other %smooth 
function $g$ on $X$ that is equal to $f^{true}$ when restricted to $\mathcal{M}$ and such that $\nabla_\x^\perp g(\x) \in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon]$ can be written as 
\[g(\x) = f_{\mathbf{v}}(\x) + \bar{k}(\x),  \] 
where $\bar{k}$ is a function that has the orthogonal gradient in $\x$ within $[-\epsilon,\epsilon]$ and that is $0$  on $\mathcal{M}$, i.e., 
\begin{align} k \in \mathcal{K} = \{\bar{k}  ~:~ \forall \bar{\x}\in \mathcal{M}, \bar{k}(\bar{\x}) =0 \wedge \nabla_\x^\perp \bar{k}(\x)\in [-\epsilon,\epsilon] \}. 
\label{Eqn:KernelFunctions}
\end{align}
 %\LL{I modified, need to double check tomorrow. Modification is to prove this kernel also for non-smooth functions (assuming some property on the gradient of the loss).}. %\LL{A point that is not clear to me is the following: In the above we say that $\text{Ker}(\mathcal{F})$ contains all the possible smooth functions that guarantee the condition. But what about continuous, but non smooth functions? Are we assuming that the limit space of a NN is $\mathcal{C}^{\infty}$ almost surely? IF this is the case, then I totally agree with the rest of the proof, but I miss this step in the current proof. Note that in general the limit space of smooth functions can be that of continuous functions (possibly not smooth) }

Let's consider a function $f_{\mathbf{v}'}$ built similarly as $f_{\mathbf{v}}$, then we obtain that all $g'(\x)$  equal to the true function and such that $\nabla_\x^\perp g'(\x) = [\mathbf{v}'-\epsilon,\mathbf{v}'+\epsilon]$ can be written as
\[g'(\x) = f_{\mathbf{v}'}(\x) + \bar{k}(\x),  \] 
with $\bar{k} \in \mathcal{K}$, where $\mathcal{K}$ is as in Equation \eqref{Eqn:KernelFunctions}. It then follows that the sets $F_{\mathbf{v}}$ and $F_{\mathbf{v}'}$ %$$F_{\mathbf{v}} = \{g \in \mathcal{F}~|~\text{almost surely }\forall \bar{\x} \in , \, g(\bar{\x})=f^{true}(\bar{\x}) \wedge \nabla_\x^\perp g(\x) = \mathbf{v}\}$$
%$$F_{\mathbf{v}'} = \{g \in \mathcal{F} ~|~\text{almost surely }\forall \bar{\x} \in ,\,  g(\bar{\x})=f^{true}(\bar{\x}) \wedge \nabla_\x^\perp g(\x) = \mathbf{v}'\}$$
are such that $F_{\mathbf{v}}=F_{\mathbf{v}'}+(f_{\mathbf{v}}-f_{\mathbf{v}'}). $ 
%Hence, because the prior is invariant to translations\footnote{Note that similarly than how shown for sets $F_{\mathbf{v}}$, $F_{\mathbf{v'}}$ it can be shown that sets $G_{\mathbf{v}}=\{g\in \mathcal{F} : \nabla_\x^\perp g(\x) \in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon] \}$, $G_{\mathbf{v'}}=\{g\in \mathcal{F} : \nabla_\x^\perp g(\x) \in [\mathbf{v}'-\epsilon,\mathbf{v}'+\epsilon] \}$ are equal up to a translation.} (see Definition \ref{Def:UninformativePrior}) and the likelihood is the same for both sets of functions (each function is equal to the true function), we obtain that these sets have same posterior measure.
Hence, $P(\nabla_\x^\perp f(\x)\in [\mathbf{v}-\epsilon,\mathbf{v}+\epsilon] \mid D_\infty)=P(\nabla_\x^\perp f(\x)\in [\mathbf{v}'-\epsilon,\mathbf{v}'+\epsilon] \mid D_\infty).$ Thus, concluding the proof.

%is the same for any $\mathbf{v}(\x)$, which gives the desired result. 
%In fact, we can transform a set $F_{\mathbf{v}(\x)}$ into a set $F_{\mathbf{w}(\x)}$ by point-wise adding the function $f_{\mathbf{w}(\x)} - f_{\mathbf{v}(\x)}$ to functions in the first set. %\gc{Is this enough to state state the two sets have the same measure (an not only the same dimension)? WE NEED THE SAME MEASURE - THEY ALSO HAVE THE SAME DIMENSION - as the corresponding sets are just shifted versions of one another.}


% \iffalse
% \LL{Se serve, dovremmo essere in grado di dimostrare questa convergenza in distribuzione che assumiamo per la BNN usando il Doob's consistency theorem (Theorem 10.10 in van der Vaart, Asymptotic Statistics). Per ora non l'ho fatto perchè la cosa importante è dimostrare il resto (e poi potrebbe richiedere delle noie visto che nel nostro caso vi sono più insiemi di parametri che minimizzano la loss), e sinceramente le assunzioni abbiamo ora non mi sembrano cosi stringenti: unica assunzione che faremmo al di la della uniform prior è che convergiamo a una BNN con zero loss per infiniti dati, la cui cosa mi sembra ragionevole. }
% The operator that maps a function to its gradient is linear and bounded, thus it preserves weak convergence \citep{}. Consequently, by the Portmanteau lemma it holds that
% \begin{equation}
%       \langle\nabla_\x^\perp f(\x,\w)\rangle_{P(f(\cdot,\w)\mid {D^{n})}}\to \langle\nabla_\x^\perp f(\x)\rangle_{P(f \mid {D^{\infty})}}.
%     \end{equation}
% Then, to conclude it is enough to show that
% $$   \langle\nabla_\x^\perp f(\x)\rangle_{P(f \mid {D^{\infty})}} = 0.$$
% By definition we have
% \begin{align}
% \nonumber
%  \langle\nabla_\x^\perp f(\x)\rangle_{P(f \mid {D^{\infty})}}
%     &= \int\displaylimits \nabla_\x^\perp f(\x){p_\infty(f)}df\\
%     &=\int\displaylimits_{f:\nabla_\x^\perp f(\x)>0} \nabla_\x^\perp f(\x){p_\infty(f)}df
%     + \int\displaylimits_{f:\nabla_\x^\perp f(\x)<0} \nabla_\x^\perp f(\x){p_\infty(f)}df.
%     \label{eqn:Symmetry}
% \end{align}
% A sufficient condition for the above to be zero is that for any set $H=\{ [h^l_i,h^u_i], i\in \mathbb{N}_{\leq k} \} \subseteq \mathbb{R}^{k}$ and the negated set $-H=\{ [-h^u_i,-h^l_i], i\in \mathbb{N}_{\leq k} \} \subseteq \mathbb{R}^{k}$ it holds that 
% \begin{equation} P( A(H) | D^{\infty} )=P( A(-H) | D^{\infty} ),
% \label{eq:negate_sets}
% \end{equation}
% where  
% $$ A(H):=\{ f \text{ continuous in } \mathbb{R}^d: \nabla_\x^\perp f(\x)\in H \}. $$

% In order to prove that we first show that under an uniformative prior over the weights of the BNN for $N\to \infty$ the prior of the BNN in function space converges weakly to an uninformative distribution (i.e., a Gaussian with infinitely-wide variance). This can be done by relying on the weak convergence of BNNs to Gaussian processes. In particular, the prior distribution of the BNN in function space  converges weakly to a zero mean Gaussian process $p(f)=\mathcal{N}(f\mid 0,\Sigma^L),$ whose variance  $\Sigma^L \left(x_1,x_1\right)$ at a test point $x_1$ is iteratively defined by the set of equations \cite{lee2017deep}:
% %\ref{e}
% \begin{align}
%     \nonumber
%      \Sigma^l(x_1,x_1) &=  \sigma^2_b+\frac{\sigma^2_w}{4 } {\Sigma^{l-1}(x_1,x_1)}  
% \end{align}
% for $l = 1,\ldots,L$, where $\Sigma^0(x_1,x_1) =  \sigma^2_b+{\sigma^2_w} C_{x_1}$ with $C_{x_1}$ being a constant dependent on $x_1$. From this it follows that $p(\w)$ induces an arbitrarily flat distribution $p(f)$ in function space. 

% \LL{Bisogna stare un attimo attenti al fatto che qui abbiamo due limiti e se la prior converge in distribuzione a una uniformative prior nello spazio delle funzioni, questo di per se non garantisce che anche le posterior convergano alla stessa distribuzione. In ogni caso questa è una cosa si risolve, perchè possiamo anche fare la prova direttamente per il GP indotto da una BNN. 
% Quindi direi che ora abbiamo che la posterior di una BNN ha zero loss con probabilità 1 e tutte le funzioni continnue che hanno zero loss hanno stessa densità di probabilità. Sapendo questo può per favore qualcuno aggiungere la parte dei gradienti come suggerito da Guido?
% }


% Lastly, since the operator $$\mathcal{F}:f\mapsto\nabla_\x^\perp L(f)$$ is linear, for any $\x\in$ it holds that   $\nabla_\x^\perp L(f(\x))\in H$ if and only if $\exists! \tilde{f}\in \text{Ker}(\mathcal{F})$ and $h\in H$ such that $L(f(\x))=L(\tilde{f}(\x))+L(h(\x))$. The same reasoning holds for $-H$, therefore there is a one-to-one correspondence between $A(H)$ and $A(-H)$, and their dimension is equal to $\dim(\text{Ker}(\mathcal{F}))$. 
% \ul{MISSING PART: same dimension implies same measure wrt $P(f \mid D^{\infty})$?}

% This proves equation \ref{eq:negate_sets}.

% \lb{Lo schema secondo me qui è:\\
% 1) Introduce $\mathcal{F}$ and show that a function with zero loss and prescribed orthogonal gradient of the loss can be written as $\hat{f} + k$, where $k$ is a function from the kernel of $\mathcal{F}$. \\
% 2) Show that the previous implies that all sets which are counterimage of a orthogonal gradient function have the same measure (due to the posterior being flat).\\
% 3) Work out the integral 
% \[\langle\nabla_\x^\perp f(\x)\rangle_{P(f \mid {D^{\infty})}}
%     = \int\displaylimits \nabla_\x^\perp f(\x){p_\infty(f)}df,\]
% observing that we can rewrite it as 
% \[\int_{\theta,r} \displaylimits \x(\theta,r){p_\infty(\mathcal{F}^{-1}(\x(\theta,r)))}d\theta dr \]
% where $\x(\theta,r)$ is the vector in $\mathbb{R}^d$ for a fixed $\x$ (notation to be changed) defined by the angle $\theta$ and the radius $r$.
% Now, by the previous arguments, $p_\infty$ is uniform in $\theta$. So we can normalize $\x(\theta,r)$, and integrate the unit vector over the sphere  $S^{d-1}$, which gives zero. 
% % }

% \fi

\end{proof}




% \iffalse

% \newpage



% \begin{theorem}\label{thm:main}
%     Let $\subset \mathbb{R}^d$ be a smooth data manifold and let $f(\cdot,\w)$ be a BNN trained on $$ with cross entropy loss function $L$. Assume that:
%     \begin{enumerate}[a)]
%         \item The prior distribution $p(\w)$ is uninformative.
%         \item $f(\cdot, \w)$ is infinitely-wide.
%     \end{enumerate}
%     Then, for any $\x\in$ it holds that
%     \begin{equation}
%       \langle\nabla_\x^\perp L(\x,\w)\rangle_{p\left(\w\vert D\right)}=0.
%     \label{eq:expected_gradient}
%     \end{equation}
% \end{theorem}

% \begin{proof}
% Let $\eta\in \mathbb{N}$ be the dimension of the last hidden layer of $f$. Then, to prove the statement, it is sufficient to show that for any $\epsilon>0$, there exists $\eta^*\in\mathbb{N}$ such that for all $\eta>\eta^*$ it holds that $|\langle\nabla_\x^\perp L(\x,\w)\rangle_{p\left(\w\vert D\right)}|_{\infty}<\epsilon.$

% By definition we have
% \begin{align}
% \nonumber
%  & \langle\nabla_\x^\perp L(\x,\w)\rangle_{p\left(\w\vert D\right)}
%      = \int\displaylimits_\w \nabla_\x^\perp L(\x,\w){p(\w|D)}d\w\\
%     & =\int\displaylimits_{\w:\nabla_\x^\perp L(\x,\w)>0} \nabla_\x^\perp L(\x,\w){p(\w|D)}d\w 
%     + \int\displaylimits_{\w:\nabla_\x^\perp L(\x,\w)<0} \nabla_\x^\perp L(\x,\w){p(\w|D)}d\w. 
%     \label{eqn:Symmetry}
% \end{align}

% Let $l_L=\inf_{\w} \{|\nabla_\x^\perp L_i(\x,\w)|:i=1,...,n \text{ and } \nabla_\x^\perp L_i(\x,\w)\neq 0 \}$
% be the smallest non-null absolute value of the components in $\nabla_\x^\perp L(\x,\w)$. For any fixed $0< \epsilon <\min(1,l_L)$ consider $\bar{\epsilon}:=\epsilon\,\inf_{\w: p(\w|D)>0}p(\w|D) $ and call  ${\mathbf{i}_{\epsilon}}$ the vector whose components are all equal to $\epsilon.$ 
% Then, by Proposition \ref{Proposition:ExtensionLemmaForNNs} we know that for any sets of weights $\w_2$ there exists $\eta^*$ such that if the dimension of the last layer of the neural network is wider than $\eta^*$, then there exists a set of weights $\w_1$ such that
% \LL{Need to put some assumptions on the likelihood in the background}
% \begin{align}
%  \label{eqn:OrthGrad}
%   |\nabla_\x^\perp & L(\x,\w_1) + \nabla_\x^\perp L(\x,\w_2)|_{\infty}\leq  \epsilon \\
%   &|p(\w_1|D)-p(\w_2|D)|\leq \bar\epsilon,
%     \label{eqn:EqPosterior}
% \end{align}
% where Eqn \eqref{eqn:EqPosterior} holds because $\w_1$ and $\w_2$ have same prior and converging likelihood. This implies that 
% \begin{align*}
%     - \nabla_\x^\perp L(\x,\w_1) - {\mathbf{i}_{\epsilon}} \leq &\nabla_\x^\perp L(\x,\w_2) \leq - \nabla_\x^\perp L(\x,\w_1) + {\mathbf{i}_{\epsilon}}\\
%     p(\w_1|D) - \bar\epsilon &\leq p(\w_2|D) \leq p(\w_1|D) + \bar\epsilon.
% \end{align*}

% Then,  by combining Eqns \eqref{eqn:Symmetry}, \eqref{eqn:OrthGrad}, \eqref{eqn:EqPosterior}, \gc{and proposition \ref{prop:same_measure}} we obtain:


% \begin{align*}
% | \langle\nabla_\x^\perp &L(\x,\w)\rangle_{p\left(\w\vert D\right)}|_{\infty}\\
%     =&\Bigg|\int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \nabla_\x^\perp L(\x,\w_1){p(\w_1|D)}d\w_1
%     + \int\displaylimits_{\w_2:\nabla_\x^\perp L(\x,\w_2)<0} \nabla_\x^\perp L(\x,\w_2){p(\w_2|D) }d\w_2\Bigg|_\infty\\
%     \leq& \Bigg|\int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \nabla_\x^\perp L(\x,\w_1){p(\w_1|D)}d\w_1 \\
%         &\quad \quad +\int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} ({\mathbf{i}_{\epsilon}}-\nabla_\x^\perp L(\x,\w_1))({p(\w_1|D)}+\bar\epsilon)d\w_1\Bigg|_\infty\\
%     = & \Bigg| \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \mathbf{i}_{\epsilon} p(\w_1|D)d\w_1 + \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} (\mathbf{i}_{\epsilon}-\nabla_\x^\perp L(\x,\w_1)) \bar\epsilon d \w_1 \Bigg|_\infty\\
%     \leq & \Bigg| \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \mathbf{i}_{\epsilon} p(\w_1|D)d\w_1 + \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} (\mathbf{i}_{\epsilon}-\nabla_\x^\perp L(\x,\w_1)) \epsilon p(\w_1|D) d \w_1 \Bigg|_\infty\\
%     \leq & \Bigg|  \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} (1+\epsilon)\mathbf{i}_{\epsilon} p(\w_1|D)d\w_1 -  \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \epsilon \nabla_\x^\perp L(\x,\w_1) p(\w_1|D) d \w_1 \Bigg|_\infty\\
%     \leq &  (1+\epsilon) \Bigg| \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \mathbf{i}_{\epsilon} p(\w_1|D)d\w_1\Bigg|_\infty + \epsilon\, \Bigg| \int\displaylimits_{\w_1:\nabla_\x^\perp L(\x,\w_1)>0} \nabla_\x^\perp L(\x,\w_1) p(\w_1|D) d \w_1 \Bigg|_\infty\\
%     \leq& (1+\epsilon)\epsilon+\epsilon C\leq 2 C \epsilon 
% \end{align*}


% where $C$ is bounded due to the assumption of boundedness of the loss a.e. for any  set of weights $\w$. 
% Therefore, by selecting $\epsilon<\frac{\epsilon^*}{2C}$ we conclude the proof.



% \end{proof}

% \noindent
% Note that Theorem \ref{thm:main} holds independently of the number of training data. Hence, 
% by the definition of the FGSM attack (Equation \eqref{BayesFGSM}) and other gradient-based attacks, Theorem \ref{thm:main} directly implies that any gradient-based attack will be ineffective against a BNN in the limit of infinite weights,  as they will only project an input point along the data manifold, where the loss becomes constant in the limit of high accuracy. This is formalized in the following Corollary, which is a direct consequence of Theorem \ref{thm:main}.




% \begin{corollary}\label{prop:robust_bnns}
%     Under the assumptions of Theorem \ref{thm:main}, further assume that in the limit of infinite data points $p(\w|D)$ is consistent, i.e. that the loss is minimized with probability $1$:
%     \begin{align}
%         \lim_{n\to\infty} P_{\w\sim p(\w|D)} \big(L(\x,\w)=0\big)=1,
%     \end{align}
%     where $n$ is the number of training data points. Then, $$\lim_{n\to\infty}\langle\nabla_\x L(\x,\w)\rangle_{p\left(\w\vert D\right)}=0.$$

% \end{corollary}
% \begin{proof}
%     Supposing that $L$ is minimized with probability $1$, in the limit of infinite weights and infinite training data the training loss function is null along the data manifold and in particular $\nabla_\x^{||} L(\x,\w)=0$ for any $\x\in$. Therefore, for any choice of weights $\w_1, \w_2$ built according to Theorem \ref{thm:main} the gradient of the loss function vanishes in expectation, i.e.
%     $$
%     \langle\nabla_\x L(\x,\w)\rangle_{p\left(\w\vert D\right)}=\langle\nabla_\x^\perp L(\x,\w)\rangle_{p\left(\w\vert D\right)}+\langle\nabla_\x^{||} L(\x,\w)\rangle_{p\left(\w\vert D\right)}=0.
%     $$
% \end{proof}

% \fi

\noindent
%\LL{Discuss how reasonable are the assumptions of the Theorem and in particular that the fact that a BNN converges to a zero loss distribution is something expected for i.i.d. data (you can cite Van Der Wart's book)}
%\ap{Luca, I think we need to add a sentence here to connect better. Otherwise is a bit too abrupt}\LL{Better?}
The proof of Theorem \ref{thm:main} relies on two main assumptions: 1) the prior is flat, which guarantees that probabilities are invariant with respect to translations, thus allowing for perfect cancellation in expectation, 2) the limiting distribution of an infinitely-wide BNN has zero loss with probability $1$, which allows us to only focus on the set of functions that are equal to the true functions on the data manifold almost surely.
While we will discuss the implication of the flat prior assumption in Section \ref{sec:limitations}, we would like to stress in here that because of the universal approximation properties of neural networks, the second assumption in Theorem \ref{thm:main} is a standard assumption to require, as it guarantees that our posterior converges to the true function with infinitely many data.  For example, under mild assumptions, a similar requirement has been explicitly shown to hold for infinitely-wide feed-forward Bayesian neural networks with one hidden layer  \citep{lee2000consistency}.
%We stress that in the overparameterized setting with  $\mathrm{dim}\left(\right)<d$,  Lemma \ref{extension_lemma} guarantees that the set of weights that achieve zero loss is not unique. Hence, results like the Bernstein-von Mises theorem \citep{vandervaart} cannot be directly applied to prove Theorem \ref{thm:main}. 

\begin{remark}
\label{remark_bernstein}
A key aspect in the proof of Theorem \ref{thm:main} is that when the data manifold has a dimension smaller than the ambient space, then there are multiple weight sets minimizing the loss (see Lemma \ref{extension_lemma} and Figure \ref{fig:multimodality} in Appendix \ref{sec:multimodality}) and the BNN posterior averages between them achieving vanishing orthogonal gradients. Note that, if there were just one set of minimizing weights, we could have employed standard results of asymptotic statistics, such as the Bernestein von Mises (BVM) Theorem  to study the asymptotic behaviour of the BNN \citep{vandervaart}. However, a standard application of the BVM Theorem would have led  to a convergence to a Gaussian distribution centered in the maximum likelihood parameters and with vanishing variance: this would have implied that a BNN is robust if and only if also the correspondent deterministic NN with fixed (deterministic) weights is robust, which we know not to be the case. 
\end{remark}


\begin{figure}[ht]
\centering
\includegraphics[width=1. \columnwidth]{Figures/halfMoons_final_hmc_100.png}
\caption{
%\LL{In the Figures, in the partial derivatives, notation should be $\langle\cdot \rangle_{p\left(\mathbf{w}\vert D\right)}$ and not $\langle\cdot \rangle_{\mathbf{w}}$. Same comments also for Figure 1,2, and 3. }
Expected loss gradients components on 100 two-dimensional test points from the Half Moons dataset \citep{halfmoons} (both partial derivatives of the loss function are shown). 
We used a collection of HMC BNNs, by varying the number of hidden neurons (a different number in each subplot) and training points (different color and size of dots). Each dot represents a different NN. %\ap{It is not clear that each plot is a different number of neurons , it might be worth it either updating the titles, or the caption to explain that.}\gc{agree, thanks}  
Only models with test accuracy greater than 80\% were taken into account.}
\label{fig:half_moons_hmc}
\end{figure}

==> Sections/notation_table.tex <==

\begin{table}[ht]
\centering

\begin{tabular}{l||p{9cm}}
 %\multicolumn{3}{c}{\textbf{Notation}}\\
  \textbf{Notation} & \textbf{Description} \\
  \toprule
    $X \subset \mathbb{R}^d$ & Ambient space \\
    $\mathcal{M}\subset X$ & Smooth closed data manifold \\
    $\x\in \mathcal{M}$ & Data point in the ambient space\\
    $\w\in\mathbb{R}^{n_\w}$ & Vector of weights and biases in the Neural Network \\
    $f^{true}:\mathcal{M}\to\mathbb{R}^k$ & Target function \\
    $f:\mathcal{M}\times\mathbb{R}^{n_\w}\to\mathbb{R}^k$ & Neural Network with $M$ layers and $n_m$ neurons in each layer (Sec. \ref{sec:overparameterizeD_Nns})\\
    \hline
    $f^\infty:\mathcal{M}\to\mathbb{R}^k$ & Infinitely wide function (Def. \ref{def:infiniteNN})\\
    $\mathcal{F}$ & Set of infinitely wide limit functions for the sequence $\{f_{n_M}(\x,\w)\}_{n_M>0}$\\
    $D = \{(\x_i,y_i)\}_{i=1,\ldots,n_D} $ & Set of training points $\x\in\mathcal{M}$ and labels $y\in\{1,\ldots,k\}$\\
    $L(\x,\w)=\ell(f(\x,\w), f^{true}(\x))$ & Training loss function\\
    $\{D_N\}_{N>0}$ & Sequence of datasets with increasing size $N$ \\
    $f^\infty_{D_N}$ & Infinitely wide NN trained on $D_N$ until convergence\\
    \hline
    $p(\w)$ & Prior distribution over $\w$ \\
    $p(D)$ & Data distribution \\
    $p(D|\w)$ & Likelihood of $D$ given $\w$\\
    $p(\w|D)$ & Posterior distribution over $\w$\\
    $f(\x^*|D)= \langle f(\mathbf{x},\mathbf{w})\rangle_{p\left(\mathbf{w}\vert D\right)}$ & Posterior predictive distribution at $x^*\in X$ (Eq. \ref{predDist})\\
    \hline
    $\Omega\subset\mathbb{R}^{n_\w}$ & Set of weights in the BNN\\ 
    $f: \mathbb{R}^d \times \Omega \rightarrow \mathbb{R}^k$& Bayesian Neural Network with weights $\w\in\Omega$\\
    $p(f)=\mathcal{N}(f|0,K^L)$ & Gaussian process on the space of smooth functions $f:\mathbb{R}^d\to\mathbb{R}^k$\\
    $p(f(\cdot,\w)|D_N)$ & Posterior distribution of the BNN trained on $D_N$\\
    \hline
    $T_\x\mathcal{M}$ & Tangent space to a manifold $\mathcal{M}$ at a point $\x\in\mathcal{M}$\\
    $T_\x\mathcal{M}^\perp$ & Orthogonal complement of $T_\x\mathcal{M}$ in $\x$\\
    $\nabla_{\mathbf{x}}L(\mathbf{x},\mathbf{w})$ & Gradient of the loss function $L$ w.r.t. the input $\x$\\
    $\tilde{\x}=\mathbf{x}+\epsilon\,\mathrm{sgn}\;\langle\nabla_{\mathbf{x}}L(\mathbf{x},\mathbf{w})\rangle_{p\left(\mathbf{w}\vert D\right)}$ & FGSM adversarial attack on the posterior predictive distribution (Eq. \ref{BayesFGSM})\\
 \bottomrule
\end{tabular}
\caption{
}
\label{table:notation}
\end{table}

